On the Sensing Performance of FMCW-based Integrated Sensing and Communications with Arbitrary Constellations

Integrated sensing and communications (ISAC) is expected to play a major role in numerous future applications, e.g., smart cities. Leveraging native radar signals like the frequency modulated continuous wave (FMCW) waveform additionally for data transmission offers a highly efficient use of valuable physical radio frequency (RF) resources allocated for automotive radar applications. In this paper, we propose the adoption of higher-order modulation formats for data modulation onto an FMCW waveform and provide a comprehensive overview of the entire signal processing chain. We evaluate the impact of each component on the overall sensing performance. While alignment algorithms are essential for removing the information signal at the sensing receiver, they also introduce significant dispersion to the received signal. We analyze this effect in detail. Notably, we demonstrate that the impact of non-constant amplitude modulation on sensing performance is statistically negligible when the complete signal processing chain is considered. This finding highlights the potential for achieving high data rates in FMCW-ISAC systems without compromising the sensing capabilities.

==> fmcw_block.tex <==


\tikzset{
    ultra thin/.style= {line width=0.1pt},
    very thin/.style=  {line width=0.2pt},
    thin/.style=       {line width=0.4pt},%
    semithick/.style=  {line width=0.6pt},
    thick/.style=      {line width=0.8pt},
    very thick/.style= {line width=1.2pt},
    ultra thick/.style={line width=1.6pt}
}


    \tikzstyle{bl} = [draw, line width=1pt, rectangle, inner sep=.5em, rounded corners, fill=kit-cyanblue30, font=\footnotesize]
    \tikzstyle{bl_white} = [draw, line width=1pt, rectangle, inner sep=.5em, rounded corners, font=\footnotesize]
    \tikzstyle{bl2} = [draw, very thick, circle, inner sep=.8em]
     \tikzstyle{input} = [coordinate]
     \tikzstyle{output} = [coordinate]
     \tikzstyle{every node}=[line width=1pt, font=\footnotesize]
     \tikzstyle{dot}=[circle,fill,draw,inner sep=0pt,minimum size=2pt]
    \tikzstyle{sum}=[draw, circle, minimum size=10pt]

\begin{circuitikz}[auto, line width=1pt, x=0.17cm,y=0.35cm]
    
    \node[oscillator, line width=0.6pt, scale=0.4, name=input]{};

    \node[left=1.6 of input, align=center]{$s(t)$};
   
 
    \node[circulator, right=6 of input, line width=0.6pt, scale=0.5, name=circ]{};

    \node[bareantenna,line width=0.6pt, scale=0.4, above= 0.4 of circ, name=ant_out] {};

    \node[right=0.25 of ant_out]{Tx};
    \node[bareantenna, line width=0.6pt, scale=0.4, right =4 of ant_out, name= ant_in]{};
    \node[right=0.3 of ant_in]{Rx};
    \node[mixer, line width=0.6pt, scale=0.45, below=3 of ant_out,name=mix]{};
    \node[bl_white, left=4.5 of mix, align=center, name=lp](lp){Lowpass \\ filter};
    \node[bl_white, left= 6 of lp,name=f_est, align=center]{Frequency \\ estimation};
    \node[bl_white, left=6 of f_est, name=fmcw_process, align=center]{FMCW\\processing};
    \node[left=4 of fmcw_process, name=output]{$\hat{r}$};

    \draw[arrows = {-Latex[width = 1.5mm]}] (input) to [short] (circ)(circ)--(ant_out)
    (circ)--(mix)
    (ant_in)|-node[below]{$r(t)$}(mix);
    \draw[arrows = {-Latex[width = 1.5mm]}] (mix)--(lp);
    \draw[arrows = {-Latex[width = 1.5mm]}] (lp)--node[below]{$s_\mathrm{IF}(t)$}(f_est);
    \draw[arrows = {-Latex[width = 1.5mm]}] (f_est)-- node[below]{$\hat{f}_\mathrm{b}$}(fmcw_process);
    \draw[arrows = {-Latex[width = 1.5mm]}]  (fmcw_process) --(output);    

    
       
    \end{circuitikz}


==> signals2.tex <==
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\definecolor{mycolor1}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor2}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor3}{rgb}{1.00000,0.44700,0.74100}%
\definecolor{mycolor4}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{kit-green100}{rgb}{0,.59,.51}

 

\definecolor{kit-green100}{rgb}{0,.59,.51}
\definecolor{kit-green70}{rgb}{.3,.71,.65}
\definecolor{kit-green50}{rgb}{.50,.79,.75}
\definecolor{kit-green30}{rgb}{.69,.87,.85}
\definecolor{kit-green15}{rgb}{.85,.93,.93}
\definecolor{KITgreen}{rgb}{0,.59,.51}

 

\definecolor{KITpalegreen}{RGB}{130,190,60}
\colorlet{kit-maigreen100}{KITpalegreen}
\colorlet{kit-maigreen70}{KITpalegreen!70}
\colorlet{kit-maigreen50}{KITpalegreen!50}
\colorlet{kit-maigreen30}{KITpalegreen!30}
\colorlet{kit-maigreen15}{KITpalegreen!15}

 

\definecolor{KITblue}{rgb}{.27,.39,.66}
\definecolor{kit-blue100}{rgb}{.27,.39,.67}
\definecolor{kit-blue70}{rgb}{.49,.57,.76}
\definecolor{kit-blue50}{rgb}{.64,.69,.83}
\definecolor{kit-blue30}{rgb}{.78,.82,.9}
\definecolor{kit-blue15}{rgb}{.89,.91,.95}

 

\definecolor{KITyellow}{rgb}{.98,.89,0}
\definecolor{kit-yellow100}{cmyk}{0,.05,1,0}
\definecolor{kit-yellow70}{cmyk}{0,.035,.7,0}
\definecolor{kit-yellow50}{cmyk}{0,.025,.5,0}
\definecolor{kit-yellow30}{cmyk}{0,.015,.3,0}
\definecolor{kit-yellow15}{cmyk}{0,.0075,.15,0}

 

\definecolor{KITorange}{rgb}{.87,.60,.10}
\definecolor{kit-orange100}{cmyk}{0,.45,1,0}
\definecolor{kit-orange70}{cmyk}{0,.315,.7,0}
\definecolor{kit-orange50}{cmyk}{0,.225,.5,0}
\definecolor{kit-orange30}{cmyk}{0,.135,.3,0}
\definecolor{kit-orange15}{cmyk}{0,.0675,.15,0}

 

\definecolor{KITred}{rgb}{.63,.13,.13}
\definecolor{kit-red100}{cmyk}{.25,1,1,0}
\definecolor{kit-red70}{cmyk}{.175,.7,.7,0}
\definecolor{kit-red50}{cmyk}{.125,.5,.5,0}
\definecolor{kit-red30}{cmyk}{.075,.3,.3,0}
\definecolor{kit-red15}{cmyk}{.0375,.15,.15,0}

 

\definecolor{KITpurple}{RGB}{160,0,120}
\colorlet{kit-purple100}{KITpurple}
\colorlet{kit-purple70}{KITpurple!70}
\colorlet{kit-purple50}{KITpurple!50}
\colorlet{kit-purple30}{KITpurple!30}
\colorlet{kit-purple15}{KITpurple!15}

 

\definecolor{KITcyanblue}{RGB}{80,170,230}
\colorlet{kit-cyanblue100}{KITcyanblue}
\colorlet{kit-cyanblue70}{KITcyanblue!70}
\colorlet{kit-cyanblue50}{KITcyanblue!50}
\colorlet{kit-cyanblue30}{KITcyanblue!30}
\colorlet{kit-cyanblue15}{KITcyanblue!15}
\definecolor{mycolor1}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor2}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor3}{rgb}{1.00000,0.44700,0.74100}%
\definecolor{mycolor4}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{kit-green100}{rgb}{0,.59,.51}

\centering
\begin{subfigure}[b]{0.55\textwidth}
   \includegraphics[width=1\linewidth]{f_inst.eps}
   \caption{1}
   \label{fig:Ng1} 
\end{subfigure}

\begin{subfigure}[b]{0.55\textwidth}
   \includegraphics[width=1\linewidth]{f_inst.eps}
   \caption{2}
   \label{fig:Ng2}
\end{subfigure}


==> signals_table.tex <==


\begin{figure*}[]
  \hspace*{-.25cm}  
\begin{tabular} {rl}
    \begin{tikzpicture}[baseline]
   
    \begin{axis}[
        width=1.5\columnwidth,
        height=0.35\columnwidth,
        axis background/.style={fill=white},
          grid=major, %
          grid style={gray!30}, %
          ylabel=$\mathrm{Symbols}$,
          y label style={at={(-0.1,0.5)}},
          enlarge x limits=false,
          enlarge y limits=false,
          xmin = 0,
          ymax = 2.5,
          ymin = -0.5,
          xticklabels={},
          ytick={0,1},
          yticklabels={$0$,$1$},
          legend columns=-1,
          legend style={at={(1,1)}, anchor=south east,  fill opacity=1, text opacity=1, column sep=0.2cm,font=\footnotesize},
          legend cell align={left},
          tick label style={font=\footnotesize},
          y label style={font=\footnotesize}
        ]
        \addplot+[mark=none, color=black, line width= 1pt]
        table[x=t,y=x,col sep=comma] {stream.csv};
        \addlegendentry{$|tx(t)|$ } 
        \addplot+[mark=none, color=KITcyanblue, line width= 1pt]
        table[x=t,y=disp,col sep=comma] {disp.csv};
        \addlegendentry{$|\tilde{tx}(t)|$ }
    \end{axis}
    \end{tikzpicture}
\\
    \begin{tikzpicture}[]
      \begin{axis}[
        width=1.5\columnwidth,
        height=0.35\columnwidth,
        axis background/.style={fill=white},
          grid=major, %
          grid style={gray!30}, %
          ylabel=$\mathrm{Symbols}$,
          y label style={at={(-0.1,0.5)}},
          enlarge x limits=false,
          enlarge y limits=false,
          xmin = 0,
          ymax = 2.5,
          ymin = -0.5,
          xticklabels={},
          ytick={0,1},
          yticklabels={$0$,$1$},
          legend columns=-1,
          legend style={at={(1,1)}, anchor=south east,  fill opacity=1, text opacity=1, column sep=0.2cm,font=\footnotesize},
          legend cell align={left},
          tick label style={font=\footnotesize},
          y label style={font=\footnotesize}
        ]
        \addplot+[mark=none, color=black, line width= 1pt]
        table[x=t,y=x,col sep=comma] {stream2.csv};
        \addlegendentry{$|tx(t)|$ } 
        \addplot+[mark=none, color=KITcyanblue, line width= 1pt]
        table[x=t,y=disp,col sep=comma] {disp2.csv};
        \addlegendentry{$|\tilde{tx}(t)|$ }
    \end{axis}
    \end{tikzpicture}
    
\end{tabular}
    \caption{Time domain signals for test signal and 64 QAM}
    \label{fig:signals}
\end{figure*} 

